Simulating realistic non-Gaussian state preparation

We consider conditional photonic non-Gaussian state preparation using multimode Gaussian states and photon-number-resolving detectors in the presence of photon loss. While simulation of such state preparation is often computationally challenging, we show that obtaining the required multimode Gaussian state Fock matrix elements can be reduced to the computation of matrix functions known as loop hafnians, and develop a tailored algorithm for their calculation that is faster than previously known methods. As an example of its utility, we use our algorithm to explore the loss parameter space for three specific non-Gaussian state preparation schemes: Fock state heralding, cat state heralding, and weak cubic-phase state heralding. We confirm that these schemes are fragile with respect to photon loss, yet find that there are regions in the loss parameter space that are potentially accessible in an experimental setting which correspond to heralded states with non-zero non-Gaussianity.

==> cutout.tex <==

%Therefore, we develop faster simulation methods for non-Gaussian state preparation.
%new and  efficient methods for calculating density matrices of the heralded states need to be developed, an example of which we now present. %We provide such a generalization by including losses and by providing an efficient method for the calculation of the density matrices of the heralded non-Gaussian states prepared using detectors with limited efficiency.
%We include light source and transmission imperfections, as well as inefficient detection, all modeled by loss and therefore straightforward to include in the Gaussian formalism since loss is a bosonic Gaussian channel. %Thus a lossy Gaussian states is also described by a vector of means $\vec \beta$ and a covariance matrix $\bm{\sigma}_Q$ (of the Glauber-Sudarshan $Q$ function see Appendix \ref{app:fockgaussian}).


%To accomplish this, we generalize the results of Refs.~\cite{hamilton2017gaussian,kruse2018detailed,quesada2018faster}

==> old_abs_and_intro.tex <==
We simulate lossy photonic single-mode non-Gaussian state preparation schemes. The states are prepared by measuring all but one of the modes of multimode Gaussian states using photon number-resolving detectors, a setting where experimental imperfections modeled by pure-loss channels can be accounted for easily. We first show that the Fock matrix elements of arbitrary multimode Gaussian states can be reduced to computing a matrix function known as the loop hafnian. Deploying tailored algorithms for structured matrices, we are able to compute efficiently these Fock matrix elements faster than previous known methods. Using this numerical toolbox we compute various figures of merit for several state preparation schemes: fidelity to the target state, success probability, and a measure of non-Gaussianity known as the Wigner logarithmic negativity. We find that the states are very fragile to photon loss; however, there are regions in the loss parameter space that are potentially accessible in an experimental setting which correspond to output states with non-zero Wigner log negativity. Our analysis points to the need for noise-optimized state preparation and practical non-Gaussian state distillation protocols to harness the non-Gaussianity for fault-tolerant quantum computation. %\tc{to shorten}

\section{Introduction} \label{sec:intro}
\tc{Add references to balance the CV with the discrete}
Photonic quantum information processing is a branch of quantum technologies that is aimed at harnessing the quantum properties of light at their most fundamental level~\cite{perspectives}.  In particular, there has recently been considerable theoretical and experimental progress in the field of photonic quantum computation~\cite{braunstein2005quantum,weedbrook2012gaussian}, which is the focus of this article. This comprises many different aspects such as large cluster-state generation in the time~\cite{menicucci2010arbitrarily,yokoyama2013ultra,yoshikawa2016invited,2DC} and frequency domains~\cite{menicucci2008one,chen2014experimental,roslund2014wavelength}, loop-based architectures~\cite{motes2014scalable,takeda2017universal,Marek:18,qi2018linear}, gate model algorithms~\cite{hamilton2017gaussian,rebentrost2018quantum,arrazola2018quantum,arrazola2018using}, and hybrid computation~\cite{andersen2015hybrid}. In addition to quantum computation, photonic quantum technologies enable promising applications in quantum sensing~\cite{pirandola2018advances} and quantum key distribution~\cite{laudenbach2018continuous}.

An important class of photonic states are Gaussian states that can be efficiently described and analyzed mathematically \cite{weedbrook2012gaussian,serafini2017quantum}. However, it has been shown that an all-Gaussian optical scheme, i.e., an algorithm that takes Gaussian states as inputs and performs operations mapping Gaussian states to Gaussian states, including Gaussian measurements, can be efficiently simulated using classical computers~\cite{Bartlett2002b}. Therefore,  compulsory resources for performing universal photonic quantum computation are non-Gaussian states and operations \cite{Lloyd1999a}. % Hence, photonic quantum computation comes with a compulsory requirement for non-Gaussian states and operations. 
In addition, non-Gaussianity is an advantageous resource for various other quantum information processing tasks such as quantum metrology~\cite{dowling1,dowling2}, entanglement distribution~\cite{sabapathy2011robustness}, error correction~\cite{niset2009nogo}, phase estimation~\cite{adesso2009optimal}, bosonic codes~\cite{chuang1997bosonic,bosonicterhal, michael2016new, niu2018hardware,li2017cat,heeres2017implementing}, quantum communication~\cite{sabapathy2017nongaussian}, and quantum cloning \cite{ngcloning}. The experimental generation of high-quality non-Gaussian states and gates, however, remains a key challenge and is of much interest. 

In this work we theoretically analyze known schemes for preparing non-Gaussian states in the presence of photon loss. All the methods we study rely on the same high-level strategy: multimode Gaussian states are first prepared, then all but one of the modes are measured using photon-number-resolving (PNR) detectors \cite{sabapathy2018near,su1,su2}. This induces a non-Gaussian effect on the remaining mode that can be engineered to prepare a desired target state conditioned on observing a particular measurement pattern. The output state is then referred to as heralded by the measurement outcome. This specific framework for non-Gaussian state preparation allows for a custom simulation strategy based on Gaussian Boson Sampling \cite{hamilton2017gaussian, kruse2018detailed} that greatly speeds up calculations compared to methods relying on a description of the systems directly in the Fock basis. As a result, we are able to compute useful figures of merit for the state preparation schemes for a wide range of possible experimental parameters using minimal computational resources. In particular, this allows us to identify the parameter regions where the output states remain non-Gaussian even after undergoing photon loss. 

The rest of this article is organized as follows. In Sec.~\ref{sec:bg} we provide a brief introduction to the figures of merit useful for the state preparation schemes. We then describe in Sec.~\ref{num} the numerical simulation strategy we develop for the non-Gaussian state preparation. In Sec.~\ref{sec:ex} we simulate illustrative state generation schemes for three non-Gaussian states---Fock states, cat states, and weak cubic phase resource states---and obtain the above mentioned figures of merit for a wide range of relevant loss parameters. We conclude in Sec.~\ref{conc}. The explicit connection between the Fock matrix elements of Gaussian states and loop halfnians is presented in Appendix \ref{app:fockgaussian}.

==> pnm.tex <==



\section{Fock matrix elements of Gaussian states}\label{app:fockgaussian}

To obtain the matrix elements of a Gaussian state in the Fock basis we follow the same strategy of Refs. \cite{kruse2018detailed,hamilton2017gaussian}, i.e., we write the $Q$ function of the Gaussian state and the $P$ function of the operator $\ket{\bm{n}} \bra{\bm{m}}$, where $\ket{\bm{n}} \ (\bra{\bm{m}})$ are multimode Fock states kets (bras). This generalizes the result from Refs. \cite{kruse2018detailed,hamilton2017gaussian} in that it now allows for $\bm{n} \neq \bm{m}$ and also a closed form expression for Gaussian states with finite displacements. It generalizes the results from Ref. \cite{quesada2018faster} in that one can also calculate matrix elements of Gaussian \emph{mixed} states with finite displacement. 

The $Q$ function of an $\ell-$mode Gaussian state $\rho$ is \cite{cahill1969density}
\begin{align}
	Q_\rho(\vec{\alpha}) = \frac{1}{\sqrt{\det(\pi \bm{\sigma}_Q)}} \exp\left(-\frac{1}{2} (\vec \alpha - \vec \beta)^\dagger \bm{\sigma}_Q^{-1} (\vec \alpha - \vec \beta) \right),
\end{align}
where 
\begin{align}
	(\bm{\sigma}_Q)_{i,j} &= \tfrac{1}{2} \left\langle\left\{\hat \zeta_i , \hat \zeta_j^\dagger  \right\}  \right\rangle - \vec \beta_i \vec \beta_j^*+\tfrac{1}{2}\delta_{i,j}, \quad \vec \beta_i &= \langle{\hat \zeta_i\rangle},
\end{align}
$\{ \hat{x},\hat{y}\} \equiv \hat{x} \hat{y} +\hat{y} \hat{x}$ is the anti-commutator, and we define $\hat{\zeta}^T = \left( \hat a_1, \hat a_2, \ldots \hat a_\ell, \hat a_1^\dagger, \hat a_2^\dagger, \ldots, \hat a_\ell^\dagger \right)$, $\vec \alpha^T = (\alpha_1,\alpha_2,\ldots, \alpha_\ell, \alpha_1^*,\alpha_2^*,\ldots, \alpha_\ell^*)$.
We are interested in the following generic matrix element 
\begin{subequations}
\label{probn}
\begin{align}
\langle \bm{m}&|\rho|\bm{n} \rangle \nonumber \\
&= \pi^\ell \int d  \vec{\alpha} \ P_{\ket{\bm{n}} \bra{\bm{m}}}(\vec{\alpha}) \  Q_\rho(\vec{\alpha}) \label{probn:a}
\\
&=   \int d  \vec{\alpha} \prod_{s=1}^\ell \frac{\exp\left(|\alpha_s|^2 \right)}{\sqrt{n_s! m_s!}} \left( \partial_{\alpha_s}^{n_s} \partial_{\alpha_s^*}^{m_s} \delta(\alpha_s)  \delta(\alpha_s^*) \right)   \label{probn:b}
\\
& \times \frac{ (-1)^{n_s+m_s} }{\sqrt{\text{det}(\bm{\sigma}_Q)}}\exp\left(-\frac{1}{2} (\vec{\alpha}-\vec{\beta})^\dagger \bm{\sigma}_Q^{-1} (\vec{\alpha}-\vec{\beta}) \right)  \nonumber  \\
&=  \frac{1}{\sqrt{\text{det}(\bm{\sigma}_Q)}} \prod_{s=1}^\ell  \frac{\partial_{\alpha_s}^{n_s} \partial_{\alpha_s^*}^{m_s}}{\sqrt{n_s! m_s!}} \label{probn:c}
\\
& \times \left. \exp\left( \frac{\vec{\alpha}^\dagger \vec{\alpha}}{2} -\frac{(\vec{\alpha}-\vec{\beta})^\dagger \bm{\sigma}_Q^{-1} (\vec{\alpha}-\vec{\beta})}{2}   \right) \right|_{\vec \alpha=0}, \nonumber
\end{align}
\end{subequations}
where the vectors $\bm{m} = (m_1,\ldots,m_\ell)$ and $\bm{n} = (n_1,\ldots,n_\ell)$ contain non-negative integers and we have used the expression for the $P$ function of the operator $\ket{n} \bra{m}$ derived in Appendix \ref{sec:pnm} to write Eq. (\ref{probn:b}). In going from Eq. (\ref{probn:b}) to Eq. (\ref{probn:c}) we used the multidimensional extension of the well-known property of the derivative of a delta function $\int d\alpha d\alpha^* f(\alpha,\alpha^*)\partial_{\alpha}^n \delta(\alpha) \partial_{\alpha^*}^m \delta(\alpha^*) = (-1)^{n+m} \partial_{\alpha}^n \partial_{\alpha^*}^m f(\alpha,\alpha^*)$
The argument inside the exponential of Eq. (\ref{probn:c}) can be rearranged as follows
\begin{align} 
	&\vec{\alpha}^\dagger \vec{\alpha}- (\vec{\alpha}-\vec{\beta})^\dagger (\bm{\sigma}_Q)^{-1} (\vec{\alpha}-\vec{\beta})   \\
	&= \vec{\alpha}^\dagger (\mathbbm{1}_{2\ell} - \bm{\sigma}_Q^{-1}) \vec{\alpha}  -  \vec{\beta}^\dagger \bm{\sigma}_Q^{-1} \vec{\beta} %\ \nonumber \\
%&\quad 
+  \vec{\alpha}^\dagger  \bm{\sigma}_Q^{-1} \vec{\beta}+  \vec{\beta}^\dagger  \bm{\sigma}_Q^{-1} \vec{\alpha}. \nonumber
\end{align}
Note that the (hermitian-)matrix $\bm{\sigma}_Q$ and its inverse have the block structure  $\left[	\begin{smallmatrix}
		\bm{W} & \bm{Y}^* \\
		\bm{Y} & \bm{W}^* \\
	\end{smallmatrix} \right],
$
where  $\bm{W} = \bm{W} ^\dagger  \in \mathbb{C}^{\ell \times \ell}$ is Hermitian  and $\bm{Y} = \bm{Y} ^T \in \mathbb{C}^{\ell \times \ell}$ is symmetric. Motivated by this observation we define the following symmetric matrix 
\begin{align}
\bm{A} &= \bm{X}	\left(\mathbbm{1}_{2\ell} - \bm{\sigma}_Q^{-1} \right), \quad \bm{X} =  \begin{pmatrix}
	0 &  \mathbbm{1}_\ell \\
	\mathbbm{1}_\ell & 0  
\end{pmatrix} ,
\end{align}
and further simplify the linear terms in $\vec \alpha$ as
\begin{align}
  \vec{\alpha}^\dagger  \bm{\sigma}_Q^{-1} \vec{\beta} =   \vec{\beta}^\dagger  \bm{\sigma}_Q^{-1} \vec{\alpha} =   \vec \gamma^T  \vec \alpha, \text{ with }  \vec \gamma^T =   \vec{\beta}^\dagger \bm{\sigma}_Q^{-1}.
\end{align}
We obtain these simplification due to the block structure of $\bm{\sigma}_Q^{-1}$ and $\vec \alpha$; for these same reasons the vector $\vec \gamma$ also has a block structure where the second half of the components are the complex conjugate of the first half.

%\subsection{Matrix elements in the Fock basis}
We can now write the density matrix element of interest as
\begin{align}\label{eq:simple}
\langle \bm{m}|\rho|\bm{n} \rangle  &= T  \prod_{s=1}^\ell  \partial_{\alpha_s}^{n_s} \partial_{\alpha_s^*}^{m_s} \left. \exp\Big(\underbrace{\tfrac{1}{2} \vec \alpha^T \bm{A} \vec \alpha +  \vec \gamma^T  \vec \alpha}_{\equiv g(\vec \alpha)} \Big) \right|_{\vec \alpha=0},
\end{align}
where we have collected all the prefactors into
\begin{align}
T = \frac{1}{\sqrt{\text{det}(\bm{\sigma}_Q)}} \frac{1}{ \sqrt{\prod_{s=1}^\ell n_s! m_s!}} \exp\left(-\tfrac{1}{2} \vec \beta^\dagger \bm{\sigma}_Q^{-1} \vec \beta \right),
\end{align}
and used the fact that $\vec \alpha^\dagger \bm{X} = \vec \alpha^T $ and also $\bm{X}^2 = \mathbbm{1}_{2 \ell}$.

We now need to evaluate the derivatives appearing in Eq.~\eqref{eq:simple}. Let us first consider the case where $0 \leq n_s,m_s \leq 1$; the general case is considered at the end of this section. Using Eq.~\eqref{eq:simple} and Fa\`a di Bruno's generalization of the chain rule for partial derivatives (cf. Eq.~(4) of~\cite{hardy06}) for an exponential function $\exp\left(g(\vec{\alpha}) \right)$ we find
\begin{align}
\label{hardy}
\partial_{\vec \alpha_{i_1} }& \cdots \partial_{\vec \alpha_{i_K}}  \exp\left(g(\vec{\alpha})\right) = \\
&\exp\left( g(\vec{\alpha}) \right) \sum_{\pi \in \mathcal{P}[\{ {i_1},\ldots, {i_K}\}]} \prod_{B\in \pi} \left( \prod_{j \in B} \partial_{\vec \alpha_{j}}   g(\vec{\alpha}) \right). \nonumber
\end{align}
where $ \{i_1,...,i_K\} =I$ is an index set, the sum over $\pi$ runs over all partitions $\mathcal{P}[\{ {i_1},\ldots, {i_K}\}] $ of this set of indices, and $B$ runs over the ``blocks'' from that partition. For example, if the set of indices is $\{1,2,3,4\}$ then the partitions are
\begin{align}
\pi &= \{ \{1,2,3,4\}, \{1\} \{2,3,4\}, \{2\} \{1,3,4\}\\
&,\ldots , \{1,2\}\{3,4\},\ldots,  \{1\} \{2\}\{3\}\{4\}  \} \nonumber.
\end{align}
The blocks of the partition $\{1\} \{2,3,4\}$ are $\{1\}$ and $\{2,3,4\}$.\\

For our problem, the vectors $\bm{n}$ and $\bm{m}$ are what determines the index $I$. In particular recall that 
\begin{align}
	\alpha_s  = \vec \alpha_s \text{ but, } \alpha_s^* = \vec \alpha_{s+\ell},	
\end{align}
thus if $n_s=1 \ (n_s=0)$ then $s \in I \ (s \not\in I)$, similarly if $m_s=1 \ (m_s = 0)$ then $s+\ell \in I \ (s+\ell \not \in I)$. Using the fact that $g(\vec \alpha)$ is quadratic in $\vec \alpha$ we find
\begin{align}
 \partial_{\vec \alpha_k}  g(\vec{\alpha}) &=  \vec{\gamma}_k, \label{zero_disp}\\
\partial_{\vec \alpha_s} \partial_{\vec \alpha_k}  g(\vec{\alpha}) &= A_{s,k},%\\
% \partial_{\vec \alpha_l}  \partial_{\vec \alpha_s}  \partial_{\vec \alpha_k}  g(\vec{\alpha}) &= 0,
\end{align}
and that all higher order derivatives are zero. This means that only first and second order derivatives survive and the sum over partitions of the index set $\pi$ collapses to a sum where only partitions with subsets/blocks of at most size $2$ survive. If we label the vertices of a graph with the index set $I$ then the sum can also be understood as going over the single-pair matchings (SPMs) of the graph~\cite{quesada2018faster,bjorklund2018faster}. This is the set that enumerates the perfect matchings of a graph \emph{with loops}. For the index set $I$ we write it as SPM$(I)$. 

Whenever $n_s=0 \ (m_s=0)$ we are instructed to not include the integer $s \ (s+\ell)$ in the index set $I$. Thus we can construct the matrix $\bar{\bm{A}}$ obtained from $\bm{A}$ by keeping only the rows and columns labelled by the elements of $I$. Similarly we can construct $\bar{\gamma}$ from $\vec \gamma$ by keeping only the components indexed by the elements of $I$.
With this notation we can finally write 
\begin{align}
\bra{\bm{m}}\rho \ket{\bm{n}} &=  T  \prod_{s=1}^\ell  \partial_{\alpha_s}^{n_s} \partial_{\alpha_s^*}^{m_s} \left. \exp\left(\tfrac{1}{2} \vec \alpha^T \bm{A} \vec \alpha +  \vec \gamma^T  \vec \alpha \right) \right|_{\vec \alpha=0} \nonumber \\
 &=   T \sum_{\pi \in \text{SPM}(I) }	\prod_{(i,j) \in \pi } \tilde A_{i,j} = T \times  \text{lhaf}(\tilde{\bm{A}})
\end{align}
where we have defined
\begin{align}
	\tilde A_{i,j} = \begin{cases}
		\bar{A}_{i,j} &\text{ if } i\neq j,\\
		\bar{\gamma}_{i} &\text{ if } i=j,
	\end{cases}
\end{align}
and lhaf is the loop hafnian \cite{bjorklund2018faster}. Note that whenever $\bm{n} = \bm{m}$ and $\vec{\beta} = \vec \gamma = 0$ the above result reduces to the hafnian \emph{probabilities} calculated by Hamilton \emph{et al.} \cite{hamilton2017gaussian}.

Let us now consider the multiphoton case where $n_s, m_s > 1$. As was done before \cite{hamilton2017gaussian,kruse2018detailed,bradler2018graph,quesada2018faster} we just state that this case can be dealt with by introducing auxiliary modes in which $n_s$ photons in a single mode are mapped to $n_s$ single photons in $n_s$ modes. This implies that whenever $n_s$ (or $m_s$) is greater than one we just need to repeat the value $s$ (or $s+\ell$) in the index $I$ a total of $n_s$ (or $m_s$) times.



\section{The Glauber-Sudarshan function of $\ket{n}\bra{m}$}\label{sec:pnm}
Before starting with the derivation we state two useful identities. The first one was derived by Mehta \cite{mehta67diagonal} and gives the $P$ function of any operator $\rho$ as follows
\begin{align}\label{mehta}
	P_\rho(\alpha) =  e^{|\alpha|^2} \int \frac{d^2 \beta}{\pi^2} \ \langle -\beta |\rho|\beta \rangle  \	e^{|\beta|^2} \ e^{\beta^* \alpha - \beta \alpha^*}.
\end{align}
The second is simply a resolution of the identity (see Appendix 2 of Ref. \cite{barnett2002methods})
\begin{align}\label{identity}
	\int \frac{d^2 \beta }{\pi^2}	e^{\beta^* \alpha - \beta \alpha^*} = \delta(\alpha) \delta(\alpha^*).
\end{align}
Now we set $\rho = \ket{n}\bra{m}$ and find
\begin{align}
	\langle -\beta|n \rangle &= e^{-|\beta|^2/2} \frac{(-\beta^*)^n}{\sqrt{n!}},\\
	\langle m|\beta \rangle &= e^{-|\beta|^2/2} \frac{(\beta)^m}{\sqrt{m!}}.
\end{align}
We can now plug this into Eq. (\ref{mehta}) to find
\begin{align}
	P_{\ket{n}\bra{m}}(\alpha) 	 = e^{|\alpha|^2} \int \frac{d^2 \beta}{\pi^2} \ \frac{(-\beta^*)^n (\beta)^m }{\sqrt{m! n!}} \ e^{\beta^* \alpha - \beta \alpha^*}.
\end{align}
To make progress first consider the case $n=m=0$ for which we find
\begin{align}
	P_{\ket{0}\bra{0}}(\alpha) 	 = e^{|\alpha|^2} \int \frac{d^2 \beta}{\pi^2} \  e^{\beta^* \alpha - \beta \alpha^*} = \delta(\alpha) \delta(\alpha^*),
\end{align}
where we used the resolution of the identity in Eq. (\ref{identity}). Now note the following
\begin{align}
	(-\beta^*)^n (\beta)^m   e^{\beta^* \alpha - \beta \alpha^*}	 = (-1)^{n+m}  \partial^n_{\alpha} \partial^m_{\alpha^{*}} e^{\beta^* \alpha - \beta \alpha^*}.
\end{align}
Using this identity we find
\begin{align}
	P_{\ket{n}\bra{m}}(\alpha) 	 =  \frac{e^{|\alpha|^2}}{\sqrt{m! n!}}	(-1)^{n+m}  \partial^n_{\alpha} \partial^m_{\alpha^{*}} \delta(\alpha) \delta(\alpha^*),
\end{align}
which reduces to the well known result in Eq. 4.4.51 of Ref. \cite{gardiner2004quantum} when $n=m$. Also note that the $P$ function of $\ket{n}\bra{m}$ was derived in polar coordinates in Ref. \cite{sudarshan1963equivalence}; we just provide the derivation  in the $\alpha,\alpha^*$ basis for completeness.


\section{Complexity of computing Fock matrix elements}
%The heralded and non-deterministic preparation of non-Gaussian states using Gaussian states and PNRs was investigated in Ref. [Krishna's paper] for the case of perfect transmission and detectors. To generalize these results losses must be included and significantly more efficient methods for the calculation of the density matrices of the heralded states need to be developed. In this paper we provide such generalization by including losses and by providing an efficient method for the calculation of the density matrices of the heralded non-Gaussian states prepared using imperfect (non-unity efficiency) PNRs.
%The first task, to include loss and inefficient detection, is straightforward in the Gaussian formalism since loss is a Gaussian operation. Thus a lossy Gaussian states is also described by a vector of means $\vec \beta$ and a covariance matrix $\bm{\sigma}_Q$ (of the Glauber-Sudarshan $Q$ function see Appendix \ref{app:fockgaussian} ). Now we comment on the second task: 
In Appendix \ref{app:fockgaussian} we generalized the results of Refs. \cite{hamilton2017gaussian,kruse2018detailed,quesada2018faster} by showing that the matrix elements of a Gaussian state $\rho$ in the Fock basis $\langle \bm{m} | \rho | \bm{n} \rangle$, with $\bm{n} = (n_1,\ldots, n_\ell), \bm{m} = (m_1,\ldots, m_\ell)$ are given by a loop hafnian
\begin{align}
\langle \bm{m} | \rho | \bm{n} \rangle  = T \times  \text{lhaf}(\tilde{\bm{A}})
\end{align}
where we defined 
\begin{align}
\tilde A_{i,j} = \begin{cases}
\bar{A}_{i,j} &\text{ if } i\neq j,\\
\bar{\gamma}_{i} &\text{ if } i=j.
\end{cases}
\end{align}
and the matrix $\bar{\bm{A}}$  and vector $\bm{\gamma}$ are obtained from 
\begin{align}
\bm{A} &= \bm{X}	\left(\mathbbm{1}_{2\ell} - \bm{\sigma}_Q^{-1} \right), \quad \bm{X} =  \begin{pmatrix}
	0 &  \mathbbm{1}_\ell \\
	\mathbbm{1}_\ell & 0  
\end{pmatrix} , \\
\gamma^T &= \beta^\dagger \bm{\sigma}_Q 
\end{align}
by repeating rows (and columns) $s$ a total of $n_s$ times and rows (and columns) $s+\ell$ a total $m_s$ times. 

In general the hafnian (and loophafnian) is a hard to compute quantity and its complexity scales like $O(D^3 2^{D/2})$ with the size of the matrix $D$ (in our case $D = \sum_{s=1}^\ell n_s + m_s$).
However, this is a worst case scenario for generic matrices. For the purposes of this paper we are interested in the case where all but one of the $n_s$ and $m_s$ are fixed (this are the heralding modes for which also $n_s=m_s$) and the we want to know the matrix elements of a one mode conditioned on a certain click pattern in the $\ell-1$ modes. In this case it is convenient to use a better tailored formula for the (loop) hafnian that allows for faster calculation when the matrices in question has structure, in particular when there are rows and columns that are repeated. This formula, derived by R. Kan \cite{kan2008moments}, takes into account the repetitions of the different rows and columns (in our case these are $n_s$ and $m_s$) and it scales like\cite{huh2015boson} 
\begin{align}
\left(1+\tfrac{1}{2}  \sum_{s=1}^\ell ( n_s +  m_s ) \right) \left( \prod_{s=1}^\ell (1+n_s)(1+m_s)   \right).
\end{align}
As mentioned before if we are only interested in the $n_\ell, m_\ell$ matrix element of the $\ell^{\text{th}}$ mode conditioned on $n_1=m_1,\ldots,m_{\ell-1} = n_{\ell-1}$ clicks in the previous $\ell-1$ modes the complexity  as a function of the Fock numbers of the last mode scales like 
\begin{align}
A \, (B+n_\ell + m_\ell)  &(n_\ell+1)(m_\ell+1),\nonumber\\
 A = \left( \prod_{s=1}^{\ell-1} (1+n_s)   (1+m_s)   \right),& ~~ B =1+ \tfrac{1}{2}\sum_{s=1}^{\ell-1} n_s +  m_s.
\end{align}
 Thus the scaling as a function of the size of the Fock matrix element in the heralded mode is a low ($\leq 3$) degree polynomial. This should be contrasted with previous simulations where $\ell$ qudits were employed to approximate $\ell$ modes where the calculation scales like $d^\ell$ with $d$ being the dimensionality of the qudit, which would also dictate $n_\ell, m_\ell \leq d$. It should also be contrasted with a naive application of the generic (loop) hafnian formulas in which case the scaling would go like $O((\sum_{s} n_s+m_s)^3 2^{(\sum_{\ell} n_s+m_s)/2)}$, $s = 1, 2 \cdots,  \ell $. 
 
